PDBench: Evaluating Computational Methods for Protein Sequence Design

Proteins perform critical processes in all living systems: converting solar energy into chemical energy, replicating DNA, as the basis of highly performant materials, sensing and much more. While an incredible range of functionality has been sampled in nature, it accounts for a tiny fraction of the possible protein universe. If we could tap into this pool of unexplored protein structures, we could search for novel proteins with useful properties that we could apply to tackle the environmental and medical challenges facing humanity. This is the purpose of protein design. Sequence design is an important aspect of protein design, and many successful methods to do this have been developed. Recently, deep-learning methods that frame it as a classification problem have emerged as a powerful approach. Beyond their reported improvement in performance, their primary advantage over physics-based methods is that the computational burden is shifted from the user to the developers, thereby increasing accessibility to the design method. Despite this trend, the tools for assessment and comparison of such models remain quite generic. The goal of this paper is to both address the timely problem of evaluation and to shine a spotlight, within the Machine Learning community, on specific assessment criteria that will accelerate impact. We present a carefully curated benchmark set of proteins and propose a number of standard tests to assess the performance of deep learning based methods. Our robust benchmark provides biological insight into the behaviour of design methods, which is essential for evaluating their performance and utility. We compare five existing models with two novel models for sequence prediction. Finally, we test the designs produced by these models with AlphaFold2, a state-of-the-art structure-prediction algorithm, to determine if they are likely to fold into the intended 3D shapes.

==> relwork.tex <==

% \begin{figure*}[t]
% \centering
%   \includegraphics[width=1\linewidth]{img/data_pipeline.pdf}
%     \caption{Illustration of the data pipeline. High-quality 3D structures of proteins are obtained from a database. The side-chains of each residues are removed so to produce an empty backbone. The GNN models calculate the distances between each residue in the protein to produce a distance matrix which is used for the production of a graph. The CNN model, on the other hand, voxelises areas of space (``frame'') around each residue, with the C$\alpha$ at the center of it. Both models predict the identity of the side-chains of the residues giving a sequence of predicted residues to obtain the input 3D structure.}
%   \label{fig:data_pipeline}
% \end{figure*}


\subsubsection{Our Contributions} 
Our main contributions is the release of many open-source tools to approach the IPFP with deep learning and evaluate models for \textit{de novo} protein design. 


First, we released Aposteriori, the first open-source library to voxelise protein structures into fixed-size 3D cubes called frames.

Second, we developed TIMED (Three-dimensional Inference Method for Efficient Design), a CNN-based model which beats state-of-the-art physics-based models as well as most other deep-learning models. With this we release the full code and the model, which also include implementations for other state-of-the-art-models ProDCoNN and DenseCPD, for which code is unavailable at the time of writing.

Third, we released code to build graphs from protein structures and use GNN-based models as a novel approach to solving the IPFP. We also propose a hybrid CNN-GNN model to build on the performance of existing models and improve it. 

Finally, we created PFBench (Protein Folding Benchmark), a model-agnostic benchamrk to thoroughly evaluate and compare the biological performance of models, identify their strenghts and weaknesses, and identify potential prediction bias. We also propose the use of AlphaFold2 as a way to benchmark performance of protein design models. 

We therefore use this benchmark to evaluate state-of-the-art models for both physics-based and deep-learning-based models and compare them to identify the best-performing one for each types of proteins. 

To the best of our knowledge, we are the first ones in the field to release open-source code for protein discretisation, CNN-based models, and benchmarking, which we hope will help increasing the accessibility of the field. 

